IFC-SSL-Bench: Benchmarking Self-Supervised Learning for Annotation-Efficient Multispectral Imaging Flow Cytometry

Imaging Flow Cytometry (IFC) generates large multispectral datasets, yet the need for expert annotations bottlenecks the development of supervised deep learning models. While Self-Supervised Learning (SSL) offers a solution, its application to IFC remains fragmented and lacks systematic benchmarking. To address this, we present IFC-SSL-Bench, a modular framework for evaluating SSL in IFC. We benchmark six SSL approaches across four backbones on two heterogeneous datasets. By assessing downstream classification performance across annotation regimes of the training sets (1%-100%), we quantify annotation efficiency and identify optimal configurations for high-dimensional biological imaging. SSL matches the performance of fully supervised baselines trained on 100% of annotated data while using as little as 5% of annotations for morphological classification, with advantages in low-data regimes below 5%. Across both datasets, the contrastive approach MoCo-v2 paired with ConvNeXt backbones emerged as the top-performing configuration, with ConvNeXtV1-T best for immunological synapse classification and ConvNeXtV2-T for morphological classification. We identify a clear pattern in transfer dynamics: ImageNet initialization benefits morphological classification, consistent with its visual similarity to natural images, whereas random initialization better captures the more domain-specific immunological synapse classification. SSL elevates class-specific F1-scores by over 35 percentage points for structurally complex classes at 1% of annotated data. We synthesize these insights into a unified set of guidelines for deploying self-supervised workflows in high-throughput IFC, and release the benchmark as a resource for future work.

==> 03_Article_SupplementaryVideos.tex <==
%  CONFIGURE NEW SINGLE-PAGE FORMAT 

\onecolumn % go back to one column
\fancyhead{} % make sure we get no headers
\renewcommand{\floatpagefraction}{0.1}
\lfoot[\bSupInf]{\dAuthor}
\rfoot[\dAuthor]{\cSupInf}
\newpage

\captionsetup*{format=largeformat} % make figure legend slightly larger than in the paper
\setcounter{figure}{0} % reset figure counter for Supplementary Video Figures
%\setcounter{page}{1} % reset page count
\makeatletter 
\renewcommand{\thefigure}{SV\@arabic\c@figure} % make Figure legend start with Figure S
\makeatother

%  MAIN TEXT 
\newpage
\section*{Supplementary Videos}

\begin{SCfigure*}[50][!ht]
\includegraphics[width=0.5\linewidth]{figures/temp.png}
\caption{\textbf{This is a video of a lysosome.}\\
A typical caption would go here. We use a thumbnail version of the video file as the figure.\\
Time, seconds. Scale bar, \SI{10}{\micro\meter}.}
\label{videosupp:lysosome}
\end{SCfigure*}

==> 04_Article_SupplementaryTables.tex <==
%  CONFIGURE NEW SINGLE-PAGE FORMAT 

\onecolumn % go back to one column
\fancyhead{} % make sure we get no headers
\renewcommand{\floatpagefraction}{0.1}
\lfoot[\bSupInf]{\dAuthor}
\rfoot[\dAuthor]{\cSupInf}
\newpage

\captionsetup*{format=largeformat} % make legend slightly larger than in the paper
\setcounter{table}{0} % reset table counter for Supplementary Video Figures
%\setcounter{page}{1} % reset page count
\makeatletter 
\renewcommand{\thetable}{S\@arabic\c@table} % make Table legend start with Table S
\makeatother

%  MAIN TEXT 
\newpage
\section*{Supplementary Tables}

\bigskip

\begin{table}[!h]
    \centering
    \small
    \begin{tabular}{p{3cm}|p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm} p{2.2cm}}
        Movie & US Release Date & Director & Screenwriter(s) & Story by & Producer\\
        \hline
        Episode IV – A New Hope & May 25, 1977 & \multicolumn{3}{c}{George Lucas} & Gary Kurtz\\
        Episode V – The Empire Strikes Back & May 21, 1980 & Irvin Kershner & Leigh Brackett and Lawrence Kasdan & George Lucas & Gary Kurtz\\
        Episode VI – Return of the Jedi & May 25, 1983 & Richard Marquand & Lawrence Kasdan and George Lucas & George Lucas & Howard Kazanjian\\
    \end{tabular}
    \caption{\textbf{Original ``Star Wars'' Trilogy}\\
    Extracted from \url{https://en.wikipedia.org/wiki/List_of_Star_Wars_films}.}
    \label{supptab:st1}
\end{table}




